Towards Optimal Agentic Architectures for Offensive Security Tasks

Agentic security systems increasingly audit live targets with tool-using LLMs, but prior systems fix a single coordination topology, leaving unclear when additional agents help and when they only add cost. We treat topology choice as an empirical systems question. We introduce a controlled benchmark of 20 interactive targets (10 web/API and 10 binary), each exposing one endpoint-reachable ground-truth vulnerability, evaluated in whitebox and blackbox modes. The core study executes 600 runs over five architecture families, three model families, and both access modes, with a separate 60-run long-context pilot reported only in the appendix. On the completed core benchmark, detection-any reaches 58.0% and validated detection reaches 49.8%. MAS-Indep attains the highest validated detection rate (64.2%), while SAS is the strongest efficiency baseline at $0.058 per validated finding. Whitebox materially outperforms blackbox (67.0% vs. 32.7% validated detection), and web materially outperforms binary (74.3% vs. 25.3%). Bootstrap confidence intervals and paired target-level deltas show that the dominant effects are observability and domain, while some leading whitebox topologies remain statistically close. The main result is a non-monotonic cost-quality frontier: broader coordination can improve coverage, but it does not dominate once latency, token cost, and exploit-validation difficulty are taken into account.

==> generated/core_architecture_pairwise_delta_table.tex <==
\begin{table}[H]
\caption{Paired target-level 95\% bootstrap deltas for validated detection between architectures. Positive values mean the first architecture outperforms the second. For each target and access mode, each architecture contributes its validated-detection rate over the three model families; the reported interval bootstraps the mean delta over the 20 matched targets.}
\label{tab:core-arch-deltas}
\centering
\small
\begin{tabular}{llrr}
\toprule
\textbf{Mode} & \textbf{Comparison} & \textbf{Mean Delta} & \textbf{95\% CI} \\
\midrule
Whitebox & SAS $-$ MAS-Indep & -6.7\% & [-15.0, 0.0]\% \\
Whitebox & SAS $-$ MAS-Decent & 1.7\% & [-10.0, 15.0]\% \\
Whitebox & SAS $-$ MAS-Central & 15.0\% & [1.7, 30.0]\% \\
Whitebox & SAS $-$ MAS-Hybrid & -3.3\% & [-16.7, 6.7]\% \\
Whitebox & MAS-Indep $-$ MAS-Decent & 8.3\% & [-1.7, 20.0]\% \\
Whitebox & MAS-Indep $-$ MAS-Central & 21.7\% & [6.7, 38.3]\% \\
Whitebox & MAS-Indep $-$ MAS-Hybrid & 3.3\% & [-3.3, 10.0]\% \\
Whitebox & MAS-Decent $-$ MAS-Central & 13.3\% & [3.3, 26.7]\% \\
Whitebox & MAS-Decent $-$ MAS-Hybrid & -5.0\% & [-11.7, 1.7]\% \\
Whitebox & MAS-Central $-$ MAS-Hybrid & -18.3\% & [-33.3, -6.7]\% \\
Blackbox & SAS $-$ MAS-Indep & -20.0\% & [-33.3, -8.3]\% \\
Blackbox & SAS $-$ MAS-Decent & 8.3\% & [-5.0, 23.3]\% \\
Blackbox & SAS $-$ MAS-Central & 13.3\% & [5.0, 23.3]\% \\
Blackbox & SAS $-$ MAS-Hybrid & 1.7\% & [-11.7, 15.0]\% \\
Blackbox & MAS-Indep $-$ MAS-Decent & 28.3\% & [15.0, 45.0]\% \\
Blackbox & MAS-Indep $-$ MAS-Central & 33.3\% & [18.3, 48.3]\% \\
Blackbox & MAS-Indep $-$ MAS-Hybrid & 21.7\% & [6.7, 38.3]\% \\
Blackbox & MAS-Decent $-$ MAS-Central & 5.0\% & [-5.0, 15.0]\% \\
Blackbox & MAS-Decent $-$ MAS-Hybrid & -6.7\% & [-16.7, 5.0]\% \\
Blackbox & MAS-Central $-$ MAS-Hybrid & -11.7\% & [-21.7, -1.7]\% \\
\bottomrule
\end{tabular}
\end{table}


==> generated/expanded_architecture_results_table.tex <==
\begin{table}[t]
\caption{Architecture-level results on the completed 240-run slice over B1--4 and W1--4. Detection-any counts both \texttt{tp} and \texttt{partial}.}
\label{tab:expanded-architectures}
\centering
\small
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Architecture} & \textbf{Runs} & \textbf{Detect-any} & \textbf{Validated} & \textbf{Partial} & \textbf{Infra} & \textbf{Median TTFV} & \textbf{Cost/Valid} \\
\midrule
SAS & 48 & 64.6\% & 58.3\% & 3 & 4 & 58.4s & \$0.047 \\
MAS-Indep & 48 & 66.7\% & 60.4\% & 3 & 9 & 138.7s & \$0.134 \\
MAS-Decent & 48 & 66.7\% & 60.4\% & 3 & 5 & 143.4s & \$0.171 \\
MAS-Central & 48 & 45.8\% & 39.6\% & 3 & 8 & 115.2s & \$0.107 \\
MAS-Hybrid & 48 & 54.2\% & 50.0\% & 2 & 13 & 169.0s & \$0.136 \\
\midrule
\textbf{Overall} & \textbf{240} & \textbf{59.6\%} & \textbf{53.8\%} & \textbf{14} & \textbf{39} & \textbf{98.3s} & \textbf{\$0.120} \\
\bottomrule
\end{tabular}
\end{table}


==> generated/expanded_model_results_table.tex <==
\begin{table}[t]
\caption{Model-level results on the completed 240-run slice. Claude Opus 4 and GPT-5.2 tie on validated detection, while Kimi K2 is substantially cheaper but far less stable.}
\label{tab:expanded-models}
\centering
\small
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Model} & \textbf{Runs} & \textbf{Detect-any} & \textbf{Validated} & \textbf{Partial} & \textbf{Infra} & \textbf{Median TTFV} & \textbf{Cost/Valid} \\
\midrule
GPT-5.2 & 80 & 65.0\% & 58.8\% & 5 & 4 & 214.3s & \$0.216 \\
Claude Opus 4 & 80 & 65.0\% & 58.8\% & 5 & 1 & 70.8s & \$0.087 \\
Kimi K2 & 80 & 48.8\% & 43.8\% & 4 & 34 & 132.5s & \$0.035 \\
\midrule
\textbf{Overall} & \textbf{240} & \textbf{59.6\%} & \textbf{53.8\%} & \textbf{14} & \textbf{39} & \textbf{98.3s} & \textbf{\$0.120} \\
\bottomrule
\end{tabular}
\end{table}


==> generated/expanded_slice_breakdown_table.tex <==
\begin{table}[t]
\caption{Observability and domain breakdown on the 240-run slice. Whitebox and web remain materially easier than blackbox and binary tasks.}
\label{tab:expanded-slices}
\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Slice} & \textbf{Runs} & \textbf{Detect-any} & \textbf{Validated} & \textbf{Partial} & \textbf{Inconcl./Infra} & \textbf{Median TTFV} \\
\midrule
Whitebox & 120 & 81.7\% & 70.0\% & 14 & 22 & 94.6s \\
Blackbox & 120 & 37.5\% & 37.5\% & 0 & 75 & 115.6s \\
Web & 120 & 78.3\% & 78.3\% & 0 & 26 & 92.3s \\
Binary & 120 & 40.8\% & 29.2\% & 14 & 71 & 126.5s \\
\bottomrule
\end{tabular}
\end{table}


==> generated/expanded_target_results_table.tex <==
\begin{table}[H]
\caption{Target-level results on the completed 240-run slice. Each whitebox and blackbox cell aggregates 15 runs ($5 \times 3$ models and architectures).}
\label{tab:expanded-targets}
\centering
\scriptsize
\begin{tabular}{lclrrrrr}
\toprule
\textbf{Target} & \textbf{Domain} & \textbf{CWE} & \textbf{WB Detect-any} & \textbf{WB Validated} & \textbf{BB Detect-any} & \textbf{BB Validated} & \textbf{Infra Total} \\
\midrule
W1 & web & CWE-89 & 86.7\% & 86.7\% & 86.7\% & 86.7\% & 4 \\
W2 & web & CWE-22 & 93.3\% & 93.3\% & 80.0\% & 80.0\% & 4 \\
W3 & web & CWE-639 & 66.7\% & 66.7\% & 66.7\% & 66.7\% & 1 \\
W4 & web & CWE-1336 & 93.3\% & 93.3\% & 53.3\% & 53.3\% & 4 \\
B1 & binary & CWE-120 & 93.3\% & 0.0\% & 0.0\% & 0.0\% & 6 \\
B2 & binary & CWE-134 & 86.7\% & 86.7\% & 6.7\% & 6.7\% & 8 \\
B3 & binary & CWE-190 & 73.3\% & 73.3\% & 6.7\% & 6.7\% & 7 \\
B4 & binary & CWE-798 & 60.0\% & 60.0\% & 0.0\% & 0.0\% & 5 \\
\bottomrule
\end{tabular}
\end{table}


==> generated/pilot_case_results_table.tex <==
\begin{table}[H]
\caption{Case-level outcomes for the initial SAS pilot. All web cases were validated in both modes for all three model families; binary blackbox remained unsolved in this slice.}
\label{tab:pilot-cases}
\centering
\scriptsize
\begin{tabular}{llccc}
\toprule
\textbf{Target} & \textbf{Mode} & \textbf{GPT-5.2} & \textbf{Claude Opus 4} & \textbf{Kimi K2} \\
\midrule
W1 & whitebox & \pilotTP & \pilotTP & \pilotTP \\
W1 & blackbox & \pilotTP & \pilotTP & \pilotTP \\
W2 & whitebox & \pilotTP & \pilotTP & \pilotTP \\
W2 & blackbox & \pilotTP & \pilotTP & \pilotTP \\
B1 & whitebox & \pilotPartial & \pilotPartial & \pilotPartial \\
B1 & blackbox & \pilotInconclusive & \pilotInconclusive & \pilotInconclusive \\
B2 & whitebox & \pilotTP & \pilotTP & \pilotTP \\
B2 & blackbox & \pilotInconclusive & \pilotInconclusive & \pilotInfra \\
\bottomrule
\end{tabular}
\vspace{4pt}
\begin{flushleft}
\scriptsize Legend: \pilotTP{} = validated true positive, \pilotPartial{} = correct vulnerability class without validated exploit, \pilotInconclusive{} = no supported finding, \pilotInfra{} = infrastructure/provider failure.
\end{flushleft}
\end{table}


==> generated/pilot_model_results_table.tex <==
\begin{table}[t]
\caption{Initial 24-run SAS pilot results by model family (4 targets, 2 modes each). Detection-any counts both \texttt{tp} and \texttt{partial}; validated counts only \texttt{tp}.}
\label{tab:pilot-models}
\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Model} & \textbf{Runs} & \textbf{Detect-any} & \textbf{Validated} & \textbf{Partial} & \textbf{Median TTFV} & \textbf{Cost/Valid} \\
\midrule
GPT-5.2 & 8 & 75.0\% & 62.5\% & 1 & 113.6s & \$0.086 \\
Claude Opus 4 & 8 & 75.0\% & 62.5\% & 1 & 22.8s & \$0.039 \\
Kimi K2 & 8 & 75.0\% & 62.5\% & 1 & 58.6s & \$0.012 \\
\midrule
\textbf{Overall} & \textbf{24} & \textbf{75.0\%} & \textbf{62.5\%} & \textbf{3} & \textbf{58.6s} & \textbf{\$0.046} \\
\bottomrule
\end{tabular}
\end{table}


==> generated/pilot_slice_breakdown_table.tex <==
\begin{table}[t]
\caption{Outcome breakdown on the initial pilot slice. The dominant failure mode so far is binary blackbox analysis, where no model produced a validated finding.}
\label{tab:pilot-slices}
\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Slice} & \textbf{Runs} & \textbf{Detect-any} & \textbf{Validated} & \textbf{Partial} & \textbf{Inconcl./Infra} & \textbf{Median TTFV} \\
\midrule
Whitebox & 12 & 100.0\% & 75.0\% & 3 & 0 & 55.0s \\
Blackbox & 12 & 50.0\% & 50.0\% & 0 & 6 & 111.5s \\
Web & 12 & 100.0\% & 100.0\% & 0 & 0 & 58.5s \\
Binary & 12 & 50.0\% & 25.0\% & 3 & 6 & 58.6s \\
\bottomrule
\end{tabular}
\end{table}

